EducaSim: Interactive Simulacra for CS1 Instructional Practice

Role play is a high-impact mode of training that has demonstrated its effectiveness in improving learning outcomes. However, it is difficult to scale to teacher instruction due to its inherent dependency on providing personnel who are both trained and available to facilitate this learning environment. This poses a challenge, especially to massive online courses which may employ and aid hundreds to thousands of novice teachers. In this work, we present EducaSim: a novel framework that uses generative agents to simulate a small-group section for teachers-in-training to practice instruction. EducaSim works by implementing diverse pedagogical-based personas, actual course material, and agent-based architectures constructed for instructional practice to provide a pedagogically rich environment for teachers-in-training to engage in role play learning -- without the costly overhead that comes with it. We share our experiences with constructing and making the tool available for experimental training and preparation in a six-week CS1 course supporting 20,000 students. We found that teachers who engaged generally saw it as a positive experience. We believe that EducaSim is an important step to providing experiential teaching practice at scale for closely-defined settings and has great potential for future applications.

==> response_types.tex <==
%-- Error table ----------------------------------------------------------
\begin{table}[h]
  \centering
  \begin{tabularx}{0.8\textwidth}{|>{\bfseries}p{0.15\textwidth}|X|}
    \hline
    Error       & Description \\ 
    \hline
    guess       & The student does not seem to understand or guessed the answer. This error type is characterized by expressions of uncertainty or answers that do not seem related to the problem, the options or the target answer. \\
    \hline
    misinterpret & The student misinterpreted the question. This error type is characterized by answers that arise from a misunderstanding of the question being asked. Students may mistakenly address a subtly different question, leading to an incorrect response. \\
    \hline
    careless    & The student made a careless mistake. This error type is characterized by answers that appear to utilize the correct process but contain a small mistake, resulting in an answer that is slightly off. It reflects a lack of careful attention to detail or a minor error in an otherwise sound solution approach. \\
    \hline
    right-idea  & The student has the right idea, but is not quite there. This error type is characterized by situations where the student demonstrates a general understanding of the underlying concept or approach but falls short of executing or reaching the correct solution. \\
    \hline
    imprecise   & The student's answer is not precise enough. This error type is characterized by student answers that lack the necessary level of precision. \\
    \hline
    question    & The student asks follow-up questions by asking for clarification or digging for deeper understanding. \\
    \hline
  \end{tabularx}
  \caption{Error types and their descriptions}
\end{table}

\vspace{1em}

%-- Success table --------------------------------------------------------
\begin{table}[h]
  \centering
  \begin{tabularx}{0.8\textwidth}{|>{\bfseries}p{0.15\textwidth}|X|}
    \hline
    Success     & Description \\ 
    \hline
    short       & The student does not elaborate thinking. Responses like “Yes,” “No,” “I agree,” without further explanation. \\
    \hline
    well-formed & The student replies with thought-out answers with explanations, examples, or personal insight. \\
    \hline
    vague       & The student is unsure of their answer or lacks confidence. Provides an ambiguous response. \\
    \hline
    question    & The student asks follow-up questions by asking for clarification or digging for deeper understanding. \\
    \hline
  \end{tabularx}
  \caption{Success types and their descriptions}
\end{table}
